Velocity dispersion and dynamical mass for 270 galaxy clusters in the Planck PSZ1 catalogue

We present the velocity dispersion and dynamical mass estimates for 270 galaxy clusters included in the first Planck Sunyaev-Zeldovich (SZ) source catalogue, the PSZ1. Part of the results presented here were achieved during a two-year observational program, the ITP, developed at the Roque de los Muchachos Observatory (La Palma, Spain). In the ITP we carried out a systematic optical follow-up campaign of all the 212 unidentified PSZ1 sources in the northern sky that have a declination above $-15^\circ$ and are without known counterparts at the time of the publication of the catalogue. We present for the first time the velocity dispersion and dynamical mass of 58 of these ITP PSZ1 clusters, plus 35 newly discovered clusters that are not associated with the PSZ1 catalogue. Using Sloan Digital Sky Survey (SDSS) archival data, we extend this sample, including 212 already confirmed PSZ1 clusters in the northern sky. Using a subset of 207 of these galaxy clusters, we constrained the $M_{\rm SZ}$--$M_{\rm dyn}$ scaling relation, finding a mass bias of $(1-B) = 0.83\pm0.07$(stat)$\pm0.02$(sys). We show that this value is consistent with other results in the literature that were obtained with different methods (X-ray, dynamical masses, or weak-lensing mass proxies). This result cannot dissolve the tension between primordial cosmic microwave background anisotropies and cluster number counts in the $\Omega_{\rm M}$--$\sigma_8$ plane.

==> table/SNR_before_ebc.tex <==
\begin{table}
\small
\caption{Value of the mass bias before and after the Eddigton bias correction for the S/N bins.}
\label{table:SNR_bebc}
\centering
\begin{tabular}{ccc}
\noalign{\smallskip}
\hline\hline
\noalign{\smallskip}
S/N bin  & \multicolumn{2}{c}{$(1-B)$} \\
\cline{2-3}
\noalign{\smallskip}
  %& {Eddington bias not corrected} & {Eddington bias corrected} \\
  & {EB not corrected} & {EB corrected} \\
\hline
\noalign{\smallskip}
$ \qquad \quad S/N < 4.82$     & $1.17 \pm 0.09$ & $0.99 \pm 0.07$ \\
$4.82\leq S/N < 5.47$              & $1.22 \pm 0.07$ & $1.08 \pm 0.06$ \\
$5.47\leq S/N < 6.84$              & $0.96 \pm 0.07$ & $0.89 \pm 0.06$ \\
$\; \qquad \quad S/N \geq 6.84$ & $0.84 \pm 0.11$ & $0.84 \pm 0.11$ \\
%$4.5\geq S/N \leq 6.84$  & $0.94 \pm 0.03$ & $0.78 \pm 0.02$ \\

%thesis table (wrong)
%$ \qquad \quad S/N < 4.82$     & $1.20 \pm 0.09$ & $0.73 \pm 0.05$ \\
%$4.82\leq S/N < 5.47$              & $1.26 \pm 0.07$ & $0.85 \pm 0.05$ \\
%$5.47\leq S/N < 6.84$              & $1.00 \pm 0.07$ & $0.77 \pm 0.05$ \\
%$\; \qquad \quad S/N \geq 6.84$ & $0.87 \pm 0.05$ & $0.78 \pm 0.05$ \\
%$4.5\geq S/N \leq 6.84$  & $0.94 \pm 0.03$ & $0.78 \pm 0.02$ \\

\noalign{\smallskip}
\hline
\hline
\end{tabular}
\end{table}


==> table/comparison_literature_table.tex <==

\begin{table*}
	\tiny
	\caption{Summary of mass bias measurements from the literature according to each of its particular definitions in section~\ref{sec:comparison}.}
	\label{table:(1-b)_literature}
	\centering
	\begin{tabular}{c c c c c}
	\noalign{\smallskip}
	\hline\hline
	\noalign{\smallskip}
	\, SURVEY & REFERENCE SAMPLE & N. CLUSTERS & Mass bias & reference \\ 
	\noalign{\smallskip}
	\hline
	\hline
	\noalign{\smallskip}
	\multicolumn{5}{c}{X-RAY } \\
	\noalign{\smallskip}
	\hline
	\noalign{\smallskip}
	 & \planck{} PSZ1 & 189  & $0.8_{-0.2}^{+0.1} $ & {\cite{planck13_cat}}\\
	\noalign{\smallskip}
	\hline
	\hline
	\noalign{\smallskip}
	\multicolumn{5}{c}{VELOCITY DISPERSION } \\
	\noalign{\smallskip}
	\hline
	\noalign{\smallskip}
	 & SPT & 44 & $0.72 \pm 0.57$ & {\cite{ruel14}}  \\
	 & ACT & 21 & $1.10 \pm 0.13$ & {\cite{sifon16}} \\
	 & \planck{} PSZ2& 17 & $0.64 \pm 0.11$ & {\cite{amodeo17}} \\
	 %& \planck PSZ1 & 207 & $0.78 \pm 0.02 $ & {This work} \\
	 %& \planck PSZ1 & 207 & $0.88 \pm 0.07 $ & {This work} \\
	 & \planck{} PSZ1 & 207 & $0.83 \pm 0.07 \pm 0.02 $ & {This work} \\
	\noalign{\smallskip}
	\hline
	\hline
	\noalign{\smallskip}
	\multicolumn{5}{c}{WEAK LENSING } \\
	\noalign{\smallskip}
	\hline
	\noalign{\smallskip}
	WtG    & \planck{} PSZ1 & 38 & $0.688 \pm 0.072$ & {\cite{von_der_Linden14}} \\
	CCCP & \planck{} PSZ1 & 37 & $0.76 \pm 0.05$ & {\cite{hoekstra15}} \\
	LoCuSS  & \planck{} PSZ2 & 44   & $0.95 \pm 0.04$ & {\cite{smith16}} \\
	CS82  & ACT & 19 & $0.87 \pm 0.27$ & {\cite{battaglia16}} \\
	PSZ2LenS  & \planck{} PSZ2 & 32 & $0.76 \pm 0.08$ & {\cite{sereno17}} \\
	CLASH  & \planck{} PSZ1 & 21 & $0.73 \pm 0.10$ & {\cite{penna17}} \\
	HSC-SSP  & \planck{} PSZ2 & 5 & $0.80 \pm 0.15$ & {\cite{medezinski18}} \\
	HSC-SSP  & ACTPol & 8 & $0.74_{-012}^{+0.13}$ & {\cite{miyatake18}} \\
	\noalign{\smallskip}
	\hline
	\end{tabular}
\end{table*}



==> table/z_before_ebc.tex <==
\begin{table}
\small
\caption{Value of the mass bias before and after the Eddigton bias correction for the redshift bins. }
\label{table:z_bebc}
\centering
\begin{tabular}{ccc}
\noalign{\smallskip}
\hline\hline
\noalign{\smallskip}
redshift bin  & \multicolumn{2}{c}{$(1-B)$} \\
\cline{2-3}
\noalign{\smallskip}
  & {EB not corrected} & {EB corrected} \\
\hline
\noalign{\smallskip}
$  \qquad \quad z < 0.11$     & $0.84 \pm 0.10$ & $0.82 \pm 0.09$ \\
$0.11\leq z < 0.19$               & $1.17 \pm 0.12$ & $1.10 \pm 0.11$ \\
$0.19 \leq z < 0.34$               & $1.05 \pm 0.08$ & $0.96 \pm 0.08$ \\
$\; \qquad \quad z \geq 0.34$  & $1.19 \pm 0.07$ & $1.06 \pm 0.06$ \\
%$0.0\geq z \leq 0.34$          & $0.94 \pm 0.03$ & $0.78 \pm 0.02$ \\

%thesis table (wrong)
%$  \qquad \quad z < 0.11$     & $0.86 \pm 0.05$ & $0.76 \pm 0.04$ \\
%$0.11\leq z < 0.19$               & $1.23 \pm 0.11$ & $0.98 \pm 0.09$ \\
%$0.19 \leq z < 0.34$               & $1.07 \pm 0.08$ & $0.77 \pm 0.06$ \\
%$\; \qquad \quad z \geq 0.34$  & $1.24 \pm 0.07$ & $0.77 \pm 0.04$ \\
%$0.0\geq z \leq 0.34$          & $0.94 \pm 0.03$ & $0.78 \pm 0.02$ \\

\noalign{\smallskip}
\hline
\hline
\end{tabular}
\end{table}

